CAPRI: Context-Aware Interpretable Point-of-Interest Recommendation Framework

Point-of-Interest (POI ) recommendation systems have gained popularity for their unique ability to suggest geographical destinations with the incorporation of contextual information such as time, location, and user-item interaction. Existing recommendation frameworks lack the contextual fusion required for POI systems. This paper presents CAPRI, a novel POI recommendation framework that effectively integrates context-aware models, such as GeoSoCa, LORE, and USG, and introduces a novel strategy for the efficient merging of contextual information. CAPRI integrates an evaluation module that expands the evaluation scope beyond accuracy to include novelty, personalization, diversity, and fairness. With an aim to establish a new industry standard for reproducible results in the realm of POI recommendation systems, we have made CAPRI openly accessible on GitHub, facilitating easy access and contribution to the continued development and refinement of this innovative framework.

==> rev_comments.tex <==
% ----------------------- REVIEW 1 ---------------------

% Concerning the first point, the authors limit the presentation of the framework to a description of its main components (i.e., datasets, models, and metrics) and do not describe how the evaluation process is actually done.
% In particular, the authors mention in the abstract that they “present a fusion strategy to easily merge contextual information”, but from Section 3.3, it seems that the fusion strategy is already embedded into the RecSys algorithms. How is this integration performed?
% Moreover, from the evaluation shown in Table 2, it seems that GeoSoCa considers geographical, social, and categorical contexts, while LORE considers geographical, temporal, and social contexts. Is it a limitation of the models, or is it a user’s decision?
% Finally, as a suggestion for future works, it would be interesting to add the possibility for the users to specify their own dataset and evaluate the models on it.
% Concerning the relevance of the presented paper to the topic of the workshop, the fairness contribution seems very limited. In particular, the authors only mention that they introduced two user/item fairness metrics but do not show them in the evaluation in Table 2.
% In addition, it would have been interesting to include bias mitigation methods to evaluate how they can improve the fairness of a given RecSys.

% ----------------------- REVIEW 2 ---------------------

% While the framework is relevant and important for the POI recommendation domain, it is not suitable for the workshop as it lacks a discussion on bias or fairness.
% Although fairness is listed as one of the evaluation dimensions, the paper does not provide any insight into what fairness means in the context of the framework or give any examples (the fairness dimension is even skipped in Table 2).
% Additionally, there are no other aspects in the paper that are specifically relevant to the workshop, making it unsuitable for acceptance.

% ----------------------- REVIEW 3 ---------------------

% - does not discuss in the details the workshop topics;
% - lack of novelty (the core of the work was already published);
